EMO: Edge Model Overlays to Scale Model Size in Federated Learning

Federated Learning (FL) trains machine learning models on edge devices with distributed data. However, the computational and memory limitations of these devices restrict the training of large models using FL. Split Federated Learning (SFL) addresses this challenge by distributing the model across the device and server, but it introduces a tightly coupled data flow, leading to computational bottlenecks and high communication costs. We propose EMO as a solution to enable the training of large models in FL while mitigating the challenges of SFL. EMO introduces Edge Model Overlay(s) between the device and server, enabling the creation of a larger ensemble model without modifying the FL workflow. The key innovation in EMO is Augmented Federated Learning (AFL), which builds an ensemble model by connecting the original (smaller) FL model with model(s) trained in the overlay(s) to facilitate horizontal or vertical scaling. This is accomplished through three key modules: a hierarchical activation replay cache to decouple AFL from FL, a convergence-aware communication controller to optimize communication overhead, and an ensemble inference module. Evaluations on a real-world prototype show that EMO improves accuracy by up to 17.77% compared to FL, and reduces communication costs by up to 7.17x and decreases training time by up to 6.9x compared to SFL.

==> elo-v1.tex <==
\section{\nickname: Edge Model Overlay}
\label{sec:elo}

\input{fig/fig4}

\subsection{Overview}
\label{sec3:}
Figure~\ref{fig:4} illustrates the \nickname architecture. 
The AFT training in \nickname is typically hosted on edge servers within a local area network (LAN), alongside devices. An example of such a network topology is a university campus, where students' devices connect to the university's edge servers via the campus LAN. 
AFT in \nickname runs in parallel with the FL training and creates augmented models for the original FL model, which can be horizontally connected.
The key module in \nickname for AFT is the \textit{activation replay cache} (explained in Section~\ref{sec3:cache}), which effectively decouples AFT from the original FL training. In general, \nickname reuses the available activations stored in the \textit{activation replay cache}, eliminating the need to wait for new activations from devices.

During AFT training, activations generated by the FL model need to be transferred from devices to edge servers to update the \textit{activation replay cache}. 
The transmission in \nickname occurs within a LAN. Given the higher bandwidth of a LAN compared to a wide area network (WAN), this approach is more communication-efficient than classic SFL, which transmits activations to a cloud server via a WAN.
Additionally, the \textit{communication controller} module in \nickname further optimizes activation transfer by adjusting communication intervals (as detailed in Section~\ref{sec3:controller}).

After the completion of AFT training, both the original FL model and the augmented models trained in \nickname are sent to the cloud server for aggregation into an ensemble model. \nickname creates an ensemble model by employing both horizontal scaling (model boosting) and vertical scaling (model bagging) on the cloud server (as detailed in Section~\ref{sec3:assemble}). The number of models trained in AFT depends on the number of edge servers in \nickname.

\input{fig/fig5}
\subsection{Activation Replay Cache}
\label{sec3:cache}
The first key module in \nickname is the \textit{activation replay cache}, which functions to decouple AFT from FL training. 
In terms of forward locking observed in SFL, \nickname eliminates this issue by reusing activations received from previous communications. Classic SFL discards activations after a single use. 
For backward locking, \nickname preserves the original FL training workflow, thus avoiding backward locking.
In particular, \nickname implements two key deigns: hierarchical activation caching and activation replay with cache sampling.

\textbf{Hierarchical activation caching.}
The primary challenge in building an activation cache from previous communications is how to efficiently store activations on the edge server.
The size of the activation cache can be substantial, as it depends on the number of activations from all devices, which is determined by both the data size and the number of local training iterations.
\nickname employs a hierarchical caching architecture to mitigate the potentially large storage requirements. 
As shown in Figure~\ref{fig:3}, \nickname indexes activations by device ID and batch ID.
For each index (a device-batch ID pair), only the most recently updated activation is stored in the cache.
Additionally, \nickname builds a first-level activation cache on disk, which contains all activations, while maintaining a second-level GPU memory cache generated by a sampling policy.
This hierarchical activation caching architecture allows \nickname to store all activations on storage-rich disks while minimizing the I/O overhead associated with transferring activations from disk to GPU memory.

\textbf{Activation replay with cache sampling.}
The second key consideration in the \textit{activation replay cache} module is how to update the second-level GPU cache.  
In \nickname, this update process involves sampling activations from the disk cache to the GPU cache.
Specifically, after each training iteration using activations stored in the GPU cache, the cache is refreshed by sampling new activations from the disk cache.
\nickname employs a mixed sampling policy: newly received activations that haven't been loaded into the GPU cache are directly selected for training, ensuring the prioritization of fresh data. If no new activations are available (i.e., all activations have previously been loaded into the GPU cache), a random sampling strategy is used.
This policy prioritizes new activations and switches to uniform sampling once all have been utilized. Notably, the random sampling policy in \nickname can be replaced with importance sampling, where activations are selected based on their associated training loss~\cite{katharopoulos2018not}.

\subsection{Convergence-aware Communication Controller }
\label{sec3:controller}
To further minimize communication overhead, \nickname incorporates a \textit{convergence-aware communication controller} to manage activation transfer intervals. Specifically, \nickname monitors activation convergence and dynamically adjusts the frequency of communication based on convergence states of activations.

\textbf{Activation Convergence.}
Recent studies have demonstrated that, during model training, the initial (or lower) layers tend to converge earlier than the later (or upper) layers—a phenomenon referred to as the bottom-up learning dynamic~\cite{raghu2017svcca, morcos2018insights}.
This observation provides an opportunity for \nickname to reduce activation transfer costs by limiting the transfer of activations from the original FL model as it gradually converges.
During the early stages of training, when activations exhibit significant fluctuations, \nickname collects activations from devices more frequently and updates the disk cache accordingly. As training progresses and activations stabilize, the collection and update intervals are gradually extended, allowing \nickname to reuse the existing cache and thereby reduce communication overhead.
To assess activation convergence, \nickname employs Singular Vector Canonical Correlation Analysis (SVCCA)~\cite{raghu2017svcca}. The SVCCA score, a normalized metric ranging from 0 to 1, quantifies the correlation between two activations, with higher scores indicating greater convergence~\cite{raghu2017svcca}.


\input{algorithm1}

\textbf{Convergence-aware activation transmission protocol.}
Algorithm~\ref{algorithm1} outlines the convergence-aware activation transmission protocol implemented in the \textit{communication controller}, which dynamically adjusts activation transmission intervals based on convergence of activations. 
Before a device transfers activations for batch \((i,j)\), the controller first verifies whether the batch ID is already stored in the ID cache \(\mathbb{B}\). If the batch ID is not cached, the device must transmit this batch. Next, the controller checks the interval between the last activation transmission and the current attempt. The device sends activations \(a_{(i,j)}\) only if the predefined transmission interval has been reached; otherwise, the activations are not sent to \nickname, and the communication interval counter is incremented. Upon receiving the activation, \nickname checks whether the batch is already cached. If it is, \nickname retrieves the previously stored activation \(a_{(i,j)}^c\) and calculates the SVCCA score \(s_{(i,j)}\) between the new and cached activations. The cached activation is then updated with the new one, and the communication interval is adjusted using the equation \( i_{(i,j)} = \frac{1}{1 - s_{(i,j)}} \). 
This convergence-aware interval adaptation mechanism effectively minimizes redundant communication of similar activations while ensuring that non-trivial activation updates are transmitted.

\subsection{Ensemble inference}
\label{sec3:assemble}
After both FL and AFT training are completed, the original FL model, denoted as \(M_{FL}\), along with the augmented models \(M_{EMO}^i\) generated on edge server \(i\) by \nickname, are sent to the cloud for aggregation into an ensemble model. It is worth noting that AFT training can be performed on multiple edge servers, totaling \(N\), leading to the creation of multiple models within \nickname.

Therefore, \nickname employs two categories of model aggregation. The first is \textit{horizontal aggregation}, where the original FL model \(M_{FL}\) is horizontally connected to each augmented model \(M_{EMO}^i\), a process also known as model boosting~\cite{arpit2022ensemble}. This results in a deeper model \((M_{FL}, M_{EMO}^i)\), effectively increasing the number of layers in the original FL model \(M_{FL}\). 
The second is \textit{vertical aggregation}, where the final outputs (logits) from the \(N\) pairs of original FL models and their corresponding augmented models \((M_{FL}, M_{EMO}^i)\) are averaged before being used for class prediction. This approach is referred to as vertical aggregation or model bagging~\cite{arpit2022ensemble}.
The final ensemble model is deployed at the cloud for inference.


==> evaluation-v1.tex <==
\section{Evaluation}
\label{sec:evaluation}
We evaluated \nickname against two baselines, assessing both learning and system performance using metrics such as accuracy, communication cost, and training time.

\subsection{Experimental Setup}
%\input{fig/fig6}

\textbf{Testbed.}
We developed a three-tier prototype architecture comprising end devices, two edge servers, and a cloud server. The end devices are organized into two clusters: Raspberry Pi 4 Model B single-board computers and NVIDIA Jetson NX devices equipped with GPUs. The edge servers are powered by NVIDIA RTX 3070 Ti GPUs, while the cloud server operates on an NVIDIA P100 GPU hosted on Alibaba Cloud.
All end devices and edge servers are interconnected via a LAN with symmetrical upload/download bandwidths of 800 Mbps. Additionally, both the devices and edge servers are connected to the cloud server over a WAN, with an upload/download bandwidth of 100 Mbps.

\textbf{Baselines.}
We evaluated \nickname against two baselines: \textbf{FL:} The classic FL approach is applied in two configurations: \textbf{FL-Small}, where a smalle model is trained on devices, and \textbf{FL-Large}, where a large model is fully trained on devices. In both cases, the entire model remains on the devices during training. \textbf{SFL:} In the SFL baseline, the top seven layers of the large model are offloaded and trained on a server. We implement two SFL variants: \textbf{SFL-Cloud}, where the top layers are offloaded to a cloud server, and \textbf{SFL-Edge}, where they are offloaded to an edge server. \textbf{\nickname:} For \nickname, we implement two edge model overlays on separate edge servers, covering 40\% and 60\% of the devices, respectively.

\input{exp/tab1}
\input{exp/tab2}
\textbf{Training Setup.}
The training tasks are conducted on the CIFAR-10~\cite{krizhevsky2009learning} and CIFAR-100~\cite{krizhevsky2009learning} datasets, utilizing VGG and MobileNet~\cite{howard2017mobilenets} models, respectively. Both datasets are partitioned across devices in a non-independent and non-identically distributed (non-IID) manner using the Dirichlet distribution method~\cite{hsu2019measuring}. 
In each training round, 20 devices are randomly selected from a total of 100 devices. Training is carried out over 200 rounds with a learning rate of 0.01. The batch size is set to 16, and the aggregation method used for both FL and SFL is FedAvg~\cite{mcmahan2017communication}. 
Table~\ref{table:model_partition} summarizes the model configurations employed across different methods and datasets.

\subsection{Learning Performance}
\input{exp/exp1}

Figure~\ref{fig:4} illustrates the test accuracy curves for the baselines and \nickname. On CIFAR-10, FL-Large, SFL, and \nickname achieve higher accuracy in the early stages of training. However, on CIFAR-100, SFL and \nickname significantly outperform the FL methods during the initial training phases. In the later stages, \nickname consistently surpasses all baselines on both CIFAR-10 and CIFAR-100.
Table~\ref{table:exp1} reports the highest test accuracy achieved by \nickname and the baseline methods. On CIFAR-10, FL-Large achieves accuracy comparable to FL-Small. However, on CIFAR-100, FL-Large outperforms FL-Small by 8.71\%, demonstrating the benefits of increased model size in FL training. Across both datasets, \nickname outperforms all baselines by a considerable margin. Specifically, it achieves up to 3.29\% and 17.77\% higher accuracy than the FL methods on CIFAR-10 and CIFAR-100, respectively. Compared to SFL, \nickname improves accuracy by 2.38\% on CIFAR-10 and 1.38\% on CIFAR-100.

\subsection{System Performance}
\label{sec5:sys_per}
\textbf{Communication cost.}
The communication costs of \nickname and the four baselines for a single training round are presented in Table~\ref{table:comm}. On CIFAR-10, the size of VGG model is the primary contributor to communication overhead, requiring 0.6 GB for FL-Small and 2.91 GB for FL-Large. SFL introduces an additional 0.3 GB of communication overhead compared to FL-Small, totaling 0.9 GB, while \nickname reduces this to 0.83 GB.
For the CIFAR-100 task, where the MobileNet model is more lightweight, SFL results in the highest communication cost at 2.44 GB due to the communication of activations and gradients. In contrast, \nickname achieves a substantial reduction in communication overhead, lowering it to 0.34 GB—a 7.17$\times$ decrease compared to SFL.

\input{exp/tab3}
\input{exp/exp2}

\textbf{Training time.}
We further compare the average round training time and communication time for \nickname and the baseline methods, as illustrated in Figure~\ref{figure:5}. In both the CIFAR-10 and CIFAR-100 tasks, \nickname achieves the lowest training time.
For CIFAR-10, communication time is the dominant factor for FL-Small, FL-Large, and SFL-Cloud. However, SFL-Edge and \nickname benefit from higher bandwidth between devices and edge servers, resulting in reduced communication time. 
On CIFAR-100, communication time is not the bottleneck for FL-Small and FL-Large due to the smaller size of the MobileNet model. Nevertheless, both SFL-Cloud and SFL-Edge introduce additional communication time as a result of transferring activations and gradients to remote servers.
Overall, compared to FL and SFL, \nickname reduces round training time by up to 12.5$\times$ and 6.9$\times$, respectively.

%\textbf{\nickname Overhead}
%The computational overhead in \nickname originates from two main sources: the SVCCA computation time and the loading of the cache from disk to GPU memory. It was observed that the SVCCA computation contributes up to a X\% time overhead to the FL training on the device. However, since this process is parallelized, its impact is largely mitigated by the FL training time. 

==> fig/fig2.tex <==
\begin{figure}[tp]
        \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/fig1_1.png}
         \caption{Idle time on devices}
         \label{fig1:idle}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/fig1_1.png}
         \caption{Throughput on devices}
         \label{fig1:throughput}
     \end{subfigure}
		\caption{Forward and backward locking in SFL lead to idle times and decreased throughput.}
		\label{figure:1}
\end{figure}

==> fig/fig3.tex <==
\begin{figure}[tp]
        \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/fig1_1.png}
         \caption{Latency}
         \label{fig2:latency}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/fig1_1.png}
         \caption{Bandwidth consumption}
         \label{fig2:bandwidth}
     \end{subfigure}
		\caption{Activation and gradient communication in SFL results in increased latency and bandwidth consumption.}
		\label{figure:2}
\end{figure}

==> fig/fig6.tex <==
\begin{figure}
		\centering
		\includegraphics[width=0.5\textwidth]{fig/fig6.pdf}
		\caption{The testbeds used in the evaluation.}
		\label{fig:6}
\end{figure}

==> introduction-v1.tex <==
\section{Introduction}
Recent breakthroughs in machine learning (ML) applications, including language tasks~\cite{kaplan2020scaling} and vision tasks~\cite{liu2022swin}, underscore the critical importance of increasing the size of training datasets. Most datasets available for ML applications are centralized~\cite{villalobosposition}. However, distributed and private data stored at the network edge (e.g., mobile phones) is expected to play an increasingly important role in advancing edge intelligence~\cite{deng2020edge}. Federated Learning (FL) has emerged as a promising approach for training models on edge data while preserving user privacy~\cite{hard2018federated}.

However, FL currently faces a bottleneck in scaling up the size of the trained model. In FL training, the server assigns training tasks for the global model to devices, where the data is locally stored~\cite{mcmahan2017communication}. Therefore, the size of the model in an FL system is limited by the devices' computational resources relatively lower than that of a cloud server~\cite{zhang2022federated,khan2021federated}. For instance, cloud-level GPUs (e.g., NVIDIA A100 series) typically provide 10 to 1,000 times the FLOPS and 8 to 50 times the memory of edge-level GPUs (e.g., NVIDIA Nano series)~\cite{pfeiffer2023federated}. Such limitations in computational resources significantly restrict the size of models that can be trained in an FL system.

To enable the training of large models in FL, Split Federated Learning (SFL) has been proposed that offloads the later layers of the global model to a cloud server for training~\cite{thapa2022splitfed}. This approach allows devices to train only the initial layers of the global model, thereby reducing local computational demands. However, SFL faces two critical challenges:
(i) Computational locking: The dependency between devices and the server creates idle periods for both parties, leading to low parallel efficiency. This issue arises because devices must wait for the server's execution before proceeding to the next iteration, and vice versa, causing a bottleneck in overall system throughput (refer to Section~\ref{sec2:subsec_locking}).
(ii) High communication costs: SFL introduces substantial communication overhead between devices and the server, as frequent exchanges of activations and gradients result in significant latency and bandwidth consumption (refer to Section~\ref{sec2:subsec_comm}).

To address these challenges in SFL, we propose \nickname, the first system designed to scale model size in FL while maintaining compatibility with the classic FL framework. At its core, \nickname introduces an edge-layer overlay between the device and server layers, enabling the training of a deeper, connectable model that extends the original FL model by using its intermediate activation as input — a process we term Extending Layers Training (ELT). Unlike SFL, which introduces the original FL with sequential processing issues and high communication costs, ELT operates in parallel with FL training, seamlessly integrating without disrupting existing workflows.
To achieve this, \nickname incorporates three modules: the \textit{hierarchical activation replay cache}, the \textit{convergence-aware communication controller} and the \textit{ensemble inference module}. The \textit{hierarchical activation replay cache} enables \nickname to decouple ELT from FL training. The \textit{convergence-aware communication controller} reduces the communication costs of activation transfers for ELT. Additionally, the \textit{ensemble inference module} integrates \nickname models at the end of training.

This work makes the following contributions:
(i) We propose ELT, a novel approach that introduces a highly parallel extending layer training method compatible with FL training. The resulting model from ELT can increase the size of the FL model by being assembled on the cloud.
(ii) We develop three modules in \nickname to (a) decouple FL training and ELT, (b) control communication overhead, and (c) integrate the FL model with the ELT model at the end of training.
(iii) We implement \nickname on a device-edge-cloud testbed, demonstrating the effectiveness of \nickname in improving both learning and system performance.
%The rest of this article is organized as follows:
%Section~\ref{sec:related_work} reviews related work and identifies existing gaps.
%Section~\ref{sec:challenges} highlights the challenges of SFL systems and motivates the design of \nickname.
%Section~\ref{sec:elo} provides an overview and three key modules of \nickname.
%Section~\ref{sec:evaluation} evaluates \nickname against relevant baselines. 
%Section~\ref{sec:conclusion} concludes this paper and outlines potential directions for future work.

==> mac.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% mac.tex
%%
%% Umut A. Acar
%% Macros for adaptive computation paper.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\readarrow}{\ensuremath{\Longrightarrow}}
\newcommand{\currenttime}{\ttt{currentTime}\xspace}
\newcommand{\tags}[1]{\ensuremath{\mathsf{tags}(#1)}}
\newcommand{\weight}[1]{\ensuremath{\mathsf{weight}(#1)}}
\newcommand{\dist}[2]{\ensuremath{\delta(#1,#2)}}


\newcommand{\cutspace}{\vspace{-4mm}}

\newcommand{\bomb}[1]{\fbox{\mbox{\emph{\bf {#1}}}}}

\newcommand{\myparagraph}[1]{\smallskip \noindent{\bf {#1}.}}
% formatting stuff
\newcommand{\codecolsep}{1ex}



\newcommand{\rlabel}[1]{\hspace*{-1mm}\mbox{\small{\bf ({#1})}}}

\newcommand{\tablerow}{\\[5ex]}
\newcommand{\tableroww}{\\[7ex]}
\newcommand{\tableline}{
\vspace*{2ex}\\
\hline\\ 
\vspace*{2ex}}

% Don't care
\newcommand{\dontcare}{\_
}

%% filter and quicksort stuff
\newcommand{\ncf}[2]{C^{fil}_{\ensuremath{{#1},{#2}}}}
\newcommand{\ncq}[1]{C^{qsort}_{\ensuremath{#1}}}
\newcommand{\nuf}[3]{P^{fil}_{#1,(\ensuremath{{#2},{#3}})}}
\newcommand{\nuq}[2]{P^{qsort}_{(\ensuremath{{#1},{#2}})}}

%% shorthands
\newcommand{\ddg}{{\sc ddg}}
\newcommand{\ncpa}{change-propagation algorithm}
\newcommand{\adg}{{\sc adg}}
\newcommand{\nwrite}{\texttt{write}}
\newcommand{\nread}{\texttt{read}}
\newcommand{\nmodr}{\texttt{mod}}
\newcommand{\ttt}[1]{\texttt{#1}}
\newcommand{\nmodl}{\texttt{modl}}
\newcommand{\nnil}{\ttt{NIL}}
\newcommand{\ncons}[2]{\ttt{CONS({\ensuremath{#1},\ensuremath{#2}})}}
\newcommand{\nfilter}{\texttt{filter}}
\newcommand{\nfilterp}{\texttt{filter'}}
\newcommand{\naqsort}{\texttt{qsort'}}
\newcommand{\nqsort}{\texttt{qsort}}
\newcommand{\nqsortp}{\texttt{qsort'}}
\newcommand{\nnewMod}{\texttt{newMod}}
\newcommand{\nchange}{\texttt{change}}
\newcommand{\npropagate}{\texttt{propagate}}
\newcommand{\ndest}{\texttt{d}}
\newcommand{\ninit}{\texttt{init}}



%% Comment sth out. 
\newcommand{\out}[1] {}
\newcommand{\sthat}{\ensuremath{~|~}}

%% definitions
\newcommand{\defi}[1]{{\bfseries\itshape #1}}


% Code listings.
\newcounter{codeLineCntr}
\newcommand{\codeLine}
 {\refstepcounter{codeLineCntr}{\thecodeLineCntr}}
\newcommand{\codeLineL}[1]
 {\refstepcounter{codeLineCntr}\label{#1}{\thecodeLineCntr}}
\newcommand{\codeLineNN}{} %% NN = No-Number (and no change to counter)

\newenvironment{codeListing}
 {\setcounter{codeLineCntr}{0}
%  \fontsize{10}{12}
 % the first one is width the second is height
 \fontsize{9}{11}
  \fontsize{8}{8}
  \vspace{-.1in}
  \ttfamily\begin{tabbing}}
  {\end{tabbing}
   \vspace{-.1in}}

\newenvironment{codeListing8}
 {\setcounter{codeLineCntr}{0}
%  \fontsize{8}{10}
  \fontsize{8}{8}
  \vspace{-.1in}
  \ttfamily
  \begin{tabbing}}
 {\end{tabbing}
 \vspace{-.1in}
}

\newenvironment{codeListing8h}
 {\setcounter{codeLineCntr}{0}
  \fontsize{8.5}{10.5}
  \vspace{-.1in}
  \ttfamily
  \begin{tabbing}}
 {\end{tabbing}
 \vspace{-.1in}
}


\newenvironment{codeListing9}
 {\setcounter{codeLineCntr}{0}
  \fontsize{9}{11}
  \vspace{-.1in}
  \ttfamily
  \begin{tabbing}}
 {\end{tabbing}
 \vspace{-.1in}
}

\newenvironment{codeListing10}
 {\setcounter{codeLineCntr}{0}
  \fontsize{10}{12}
  \vspace{-.1in}
  \ttfamily
  \begin{tabbing}}
 {\end{tabbing}
 \vspace{-.1in}
}


\newenvironment{codeListingNormal}
 {\setcounter{codeLineCntr}{0}
  \vspace{-.1in}
  \ttfamily
  \begin{tabbing}}
 {\end{tabbing}
 \vspace{-.1in}
}

\newcommand{\codeFrame}[1]
{\begin{center}\fbox{\parbox[t]{\columnwidth}{#1}}\end{center}
% \vspace*{-.15in}
}

\newcommand{\halfBox}[1]
{\begin{center}\fbox{\parbox[t]{\columnwidth}{#1}}\end{center}
% \vspace*{-.15in}
}

\newcommand{\fullBox}[1]
{\begin{center}\fbox{\parbox[t]{\textwidth}{#1}}\end{center}
% \vspace*{-.15in}
}

%%Note this is redefined in local-mac.tex for each paper.
\newcommand{\fixedCodeFrame}[1]
{
\begin{center}
\fbox{
\parbox[t]{0.9\columnwidth}{
#1
}
}\end{center}
}

% Footnote commands.
\newcommand{\footnotenonumber}[1]{{\def\thempfn{}\footnotetext{#1}}}

% Margin notes - use \notesfalse to turn off notes.
\setlength{\marginparwidth}{0.6in}
\reversemarginpar
\newif\ifnotes
\notestrue
\newcommand{\longnote}[1]{
  \ifnotes
    {\medskip\noindent Note:\marginpar[\hfill$\Longrightarrow$]
      {$\Longleftarrow$}{#1}\medskip}
  \fi}
\newcommand{\note}[1]{
  \ifnotes
    {\marginpar{\raggedright{\tiny #1}}}
  \fi}
\newcommand{\notered}[1]{\ifnotes
    {\marginpar{\raggedright{\tiny
          {\sf\color{red} #1}}}}
    \fi}


% Stuff not wanted.
\newcommand{\punt}[1]{}

% Sectioning commands.
\newcommand{\subsec}[1]{\subsection{\boldmath #1 \unboldmath}}
\newcommand{\subheading}[1]{\subsubsection*{#1}}
\newcommand{\subsubheading}[1]{\paragraph*{#1}}

% Reference shorthands.
\newcommand{\spref}[1]{Modified-Store Property~\ref{sp:#1}}
\newcommand{\prefs}[2]{Properties~\ref{p:#1} and~\ref{p:#2}}
\newcommand{\pref}[1]{Property~\ref{p:#1}}


\newcommand{\partref}[1]{Part~\ref{part:#1}}
\newcommand{\chref}[1]{Chapter~\ref{ch:#1}}
\newcommand{\chreftwo}[2]{Chapters \ref{ch:#1} and~\ref{ch:#2}}
\newcommand{\chrefthree}[3]{Chapters \ref{ch:#1}, and~\ref{ch:#2}, and~\ref{ch:#3}}
\newcommand{\secref}[1]{{\S\ref{#1}}}
% \newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Subsection~\ref{subsec:#1}}
\newcommand{\secreftwo}[2]{Sections \ref{sec:#1} and~\ref{sec:#2}}
\newcommand{\secrefthree}[3]{Sections \ref{sec:#1},~\ref{sec:#2},~and~\ref{sec:#3}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
% \newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\figreftwo}[2]{Figures \ref{fig:#1} and~\ref{fig:#2}}
\newcommand{\figrefthree}[3]{Figures \ref{fig:#1}, \ref{fig:#2} and~\ref{fig:#3}}
\newcommand{\figreffour}[4]{Figures \ref{fig:#1},~\ref{fig:#2},~\ref{fig:#3}~and~\ref{fig:#4}}
\newcommand{\figpageref}[1]{page~\pageref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\tabreftwo}[2]{Tables~\ref{tab:#1} and~\ref{tab:#1}}

\newcommand{\stref}[1]{step~\ref{step:#1}}
\newcommand{\caseref}[1]{case~\ref{case:#1}}
\newcommand{\lineref}[1]{line~\ref{line:#1}}
\newcommand{\linereftwo}[2]{lines \ref{line:#1} and~\ref{line:#2}}
\newcommand{\linerefthree}[3]{lines \ref{line:#1},~\ref{line:#2},~and~\ref{line:#3}}
\newcommand{\linerefrange}[2]{lines \ref{line:#1} through~\ref{line:#2}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\thmreftwo}[2]{Theorems \ref{thm:#1} and~\ref{thm:#2}}
\newcommand{\thmrefthree}[3]{Theorems \ref{thm:#1}, \ref{thm:#2} and~\ref{thm:#3}}
\newcommand{\thmpageref}[1]{page~\pageref{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\lemreftwo}[2]{Lemmas \ref{lem:#1} and~\ref{lem:#2}}
\newcommand{\lemrefthree}[3]{Lemmas \ref{lem:#1},~\ref{lem:#2},~and~\ref{lem:#3}}
\newcommand{\lempageref}[1]{page~\pageref{lem:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\defreftwo}[2]{Definitions \ref{def:#1} and~\ref{def:#2}}
\newcommand{\defpageref}[1]{page~\pageref{def:#1}}
% \renewcommand{\eqref}[1]{Equation~(\ref{eq:#1})}
\renewcommand{\eqref}[1]{Equation~(\ref{#1})}
\newcommand{\eqreftwo}[2]{Equations (\ref{eq:#1}) and~(\ref{eq:#2})}
\newcommand{\eqpageref}[1]{page~\pageref{eq:#1}}
\newcommand{\ineqref}[1]{Inequality~(\ref{ineq:#1})}
\newcommand{\ineqreftwo}[2]{Inequalities (\ref{ineq:#1}) and~(\ref{ineq:#2})}
\newcommand{\ineqpageref}[1]{page~\pageref{ineq:#1}}
\newcommand{\itemref}[1]{Item~\ref{item:#1}}
\newcommand{\itemreftwo}[2]{Item~\ref{item:#1} and~\ref{item:#2}}

% Useful shorthands.
\newcommand{\abs}[1]{\left| #1\right|}
\newcommand{\card}[1]{\left| #1\right|}
\newcommand{\norm}[1]{\left\| #1\right\|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
  \renewcommand{\choose}[2]{{{#1}\atopwithdelims(){#2}}}
\newcommand{\ang}[1]{\langle#1\rangle}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\prob}[1]{\Pr\left\{ #1 \right\}}
\newcommand{\expect}[1]{\mathrm{E}\left[ #1 \right]}
\newcommand{\expectsq}[1]{\mathrm{E}^2\left[ #1 \right]}
\newcommand{\variance}[1]{\mathrm{Var}\left[ #1 \right]}
\newcommand{\twodots}{\mathinner{\ldotp\ldotp}}

% Standard number sets.
\newcommand{\reals}{{\mathrm{I}\!\mathrm{R}}}
\newcommand{\integers}{\mathbf{Z}}
\newcommand{\naturals}{{\mathrm{I}\!\mathrm{N}}}
\newcommand{\rationals}{\mathbf{Q}}
\newcommand{\complex}{\mathbf{C}}

% Special styles.
\newcommand{\proc}[1]{\ifmmode\mbox{\textsc{#1}}\else\textsc{#1}\fi}
\newcommand{\procdecl}[1]{
  \proc{#1}\vrule width0pt height0pt depth 7pt \relax}
  \newcommand{\func}[1]{\ifmmode\mathrm{#1}\else\textrm{#1}fi} %
%  Multiple cases.  
\renewcommand{\cases}[1]{\left\{
  \begin{array}{ll}#1\end{array}\right.}
  \newcommand{\cif}[1]{\mbox{if $#1$}} 

%% spacing hacks
\newcommand{\longpage}{\enlargethispage{\baselineskip}}
\newcommand{\shortpage}{\enlargethispage{-\baselineskip}}



%% Notes, todos, and remarks
\newcounter{remark}[section]

\newcommand{\myremark}[3]{
\refstepcounter{remark}
\[
\left\{
\sf 
\parbox{\columnwidth}{
{\bf {#1}'s remark~\theremark:} 
{#3}
}
\right\}
\]
%\marginpar{\bf {#2}.~\theremark}
}


% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
% For amsthm package:

%\theoremstyle{plain}
%\newtheorem{thm}{Theorem}[section]
%% \newtheorem{lem}[thm]{Lemma}
%% \newtheorem{prop}[thm]{Proposition}
%% \newtheorem*{cor}{Corollary}

%% \theoremstyle{definition}
%% \newtheorem{defn}{Definition}[section]
%% \newtheorem{conj}{Conjecture}[section]
%% \newtheorem{falseconj}{False~Conjecture}[section]
%% \newtheorem{exmp}{Example}[section]

%% \theoremstyle{remark}
%% \newtheorem*{rem}{Remark}
%% %\newtheorem*{note}{Note}
%% \newtheorem{case}{Case}


\newcommand{\uremark}[1]{\myremark{Umut}{U}{#1}}
\newcommand{\ur}[1]{\uremark{#1}}
\newcommand{\rremark}[1]{\myremark{Ruy}{R}{#1}}
\newcommand{\mremark}[1]{\myremark{Matthew}{M}{#1}}
\newcommand{\todoremark}[1]{\myremark{TODO}{TODO}{#1}}
%\newcommand{\todo}[1]{\myremark{TODO}{TODO}{#1}}
\newcommand{\todo}[1]{{\bf{[TODO:{#1}]}}}

%%

